Architecting Data-Intensive Applications : From Data Architecture Design to Its Quality Assurance

Context - The exponential growth of data is becoming a significant concern. Managing this data has become incredibly challenging, especially when dealing with various sources in different formats and speeds. Moreover, Ensuring data quality has become increasingly crucial for effective decision-making and operational processes. Data Architecture is crucial in describing, collecting, storing, processing, and analyzing data to meet business needs. Providing an abstract view of data-intensive applications is essential to ensure that the data is transformed into valuable information. We must take these challenges seriously to ensure we can effectively manage and use the data to our advantage. Objective - To establish an architecture framework that enables a comprehensive description of the data architecture and effectively streamlines data quality monitoring. Method - The architecture framework utilizes Model Driven Engineering (MDE) techniques. Its backing of data-intensive architecture descriptions empowers with an automated generation for data quality checks. Result - The Framework offers a comprehensive solution for data-intensive applications to model their architecture efficiently and monitor the quality of their data. It automates the entire process and ensures precision and consistency in data. With DAT, architects and analysts gain access to a powerful tool that simplifies their workflow and empowers them to make informed decisions based on reliable data insights. Conclusion - We have evaluated the DAT on more than five cases within various industry domains, demonstrating its exceptional adaptability and effectiveness.

==> include/1-front/titlepage.tex <==
\begin{frontespizio}
% Remember: After editing this file, delete the cache and recompile
%---------------------Definizione font---------------------%

\Preambolo{\renewcommand{\fronttitlefont}{\fontsize{22}{22}\bfseries}}
%24 24
%----------------------------------------------------------%
	% \frontinstitutionfont 	Neretto, 14/17 
	% \frontdivisionfont 		Tondo, 12/16 
	% \frontpretitlefont 		Maiuscoletto, 10/12
	% \fronttitlefont 		Neretto, 17/21 
	% \frontsubtitlefont 		Tondo, 12/14
	% \frontfixednamesfont 		Tondo, 12/14 
	% \frontnamesfont 		Neretto, 12/14 
	% \frontsmallfont 		Neretto, 9/11 
	% \frontfootfont	 	Neretto, 12/14 

	% \bfseries	Grassetto
	% \itshape	Corsivo
	% \scshape	Maiuscoletto
%----------------------------------------------------------%
\Margini{4cm}{3cm}{3cm}{3cm} % Margini sinistro, in basso, destro e in alto
\Logo[4cm]{figures/logo/UnivAQ_logoC.png}
%\Universita{L'Aquila}
\Istituzione{Dipartimento di Ingegneria e Scienze dell'Informazione e Matematica}
%\Divisione{Department of Information Engineering, Computer Science and Mathematics}	% ENG
\Divisione{Ph.D.’s Degree Thesis in Information and Communication Technologies (ICT)}		% ITA
%\Dipartimento{Dipartimento di Ingegneria e Scienze dell'Informazione e Matematica}
%\Corso[Master Degree]{Ingegneria delle Telecomunicazioni}
\Scuola{}
\Titoletto{}
\Titolo{Architecting Data-Intensive Applications : From Data Architecture Design to Its Quality Assurance}
\Sottotitolo{SSD INF/01}

\Punteggiatura{} % Modifica la punteggiatura dopo 'Candidato', 'Realatore' ecc. (vuoto per togliere)
\NCandidato{Candidate}
% {Laureando} % Sostituisce 'Candidato' con '...'
\Preambolo{\renewcommand{\frontsmallfont}[1]{\small}}
\Candidato [Student ID 270451]{Moamin B. Abughazala}
% [matricola]{Moamin B. Abughazala}

\NRelatore{Supervisor}{Relatori}
%\NRelatore{Relatore}{Relatori}
\Relatore{Prof. Henry Muccini}
% \NRelatore{Doctoral Program Supervisor}{Relatori}
% \NCorrelatore{Prof. Vittorio Cortellessa}{Relatori}
%\Correlatore{Dr. YYY YYY}
%\Rientro{1cm} % Rientro di Relatore e Candidato

\Piede{Academic Year 2021/2022}
\end{frontespizio}

\IfFileExists{\jobname-frn.pdf}{}{%
\immediate\write18{pdflatex \jobname-frn}}
